Kalyna Block Cipher: From Design Space Exploration to ASIC Design

The Kalyna block cipher is a Ukrainian cryptography standard, selected through a national competition held between 2007 and 2010 and approved in 2015. Although its software implementations have been introduced, hardware-efficient implementations of the algorithm, i.e., accelerators, do not exist. In this paper, we explore various design architectures to implement its encryption, decryption, and unified encryption/decryption functions, considering the trade-off between area and latency. We present hardware reduction techniques and introduce alternative designs with low area, latency, and energy consumption, targeting an application-specific integrated circuit (ASIC). We present hardware-efficient designs that include countermeasures against side-channel analysis (SCA) and fault injection (FI) attacks, such as hiding, masking, and duplication techniques. We validate these implementations in a 65\;nm ASIC chip. Experimental results confirm the need for alternative designs that explore the design search space for different requirements. The proposed architectures enable hiding the power SCA leakage by randomizing the execution of operations, and the temporal duplication in designs with countermeasures against the SCA attacks can mitigate the FI attacks. The functionality of the ASIC test chip, including various Kalyna designs, is validated through measurements.

==> tables <==
\begin{table}[t]
	\centering
	\caption{Parameters of the Kalyna block cipher.}
	\vspace{-3mm}
	\footnotesize
	\begin{tabular}{|c|c|c|c|}
		\hline
		Block Size ($l$) & Key Length ($k$) & \#Rounds ($t$) & \#Columns in ISM ($c$)\\ 
		\hline \hline
		\multirow{2}{*}{128}  & 128 & 10 & \multirow{2}{*}{2}  \\
		                      & 256 & 14 &                     \\
		\hline
		\multirow{2}{*}{256}  & 256 & 14 & \multirow{2}{*}{4}  \\
		                      & 512 & 18 &                     \\
		\hline
		512                   & 512 & 18 & 8                   \\
		\hline
	\end{tabular}
	\label{tab:kalyna}
	\vspace{-6mm}
\end{table}

\begin{table}[t]
	\centering
	\caption{Clock cycles in Kalyna encryption and decryption functions.}
	\vspace{-3mm}
	\footnotesize
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{Design} & \multicolumn{5}{c|}{$k/l$} \\
		\cline{2-6}
		                       & 128/128 & 128/256 & 256/256 & 256/512 & 512/512 \\ 
		\hline \hline
		parallel   & 1   & 1   & 1   & 1   & 1 \\
		serial2rnd & 5   & 7   & 7   & 9   & 9 \\
		serial1rnd & 11  & 15  & 15  & 19  & 19 \\
		serial1opr & 64  & 84  & 84  & 104 & 104 \\
		serial1col & 190 & 250 & 416 & 516 & 928 \\
		\hline
	\end{tabular}
	\label{tab:clock}
	\vspace{-6mm}
\end{table}

\begin{table*}[t]
  \centering
  \caption{Synthesis results of Kalyna designs under the \textit{serial1col} architecture.}
  \vspace{-3mm}
  \footnotesize
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{$k$} & \multirow{2}{*}{$l$} & \multicolumn{5}{c|}{Encryption} & \multicolumn{5}{c|}{Decryption} & \multicolumn{5}{c|}{Encryption \& Decryption} \\ 
    \cline{3-17}
    & & area & delay & latency & power & energy & area & delay & latency & power & energy & area & delay & latency & power & energy\\
    \hline \hline
    128 & 128 & 23662 & 4.171 & 792  & 1.191 & 944   & 35946 & 4.449 & 845  & 1.957 & 1654  & 37172  & 4.497 & 854  & 1.996 & 1705  \\
    128 & 256 & 24323 & 4.171 & 1042 & 1.186 & 1237  & 36548 & 4.433 & 1108 & 1.972 & 2185  & 37975  & 4.502 & 1125 & 2.011 & 2263  \\
    256 & 256 & 39549 & 4.285 & 1782 & 1.744 & 3109  & 55286 & 4.791 & 1993 & 2.623 & 5228  & 57673  & 4.801 & 1997 & 2.704 & 5400  \\
    256 & 512 & 41999 & 4.285 & 2211 & 1.755 & 3880  & 57553 & 4.882 & 2519 & 2.614 & 6585  & 59331  & 4.846 & 2500 & 2.680 & 6701  \\
    512 & 512 & 73966 & 4.786 & 4441 & 2.964 & 13164 & 97411 & 4.685 & 4347 & 4.122 & 17921 & 101036 & 4.658 & 4322 & 4.233 & 18298 \\		
    \hline
  \end{tabular}
  \label{tab:serial1col}
  \vspace{4.0mm}
\end{table*}

\begin{table*}[t]
  \centering
  \caption{Impact of hardware reduction techniques on the Kalyna designs under the \textit{serial1col} architecture.}
  \vspace{-3mm}
  \footnotesize
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{HRT} & \multicolumn{5}{c|}{Encryption} & \multicolumn{5}{c|}{Decryption} & \multicolumn{5}{c|}{Encryption \& Decryption} \\ 
    \cline{2-16}
    & area & delay & latency & power & energy & area & delay & latency & power & energy & area & delay & latency & power & energy\\
    \hline \hline
    KSA-OPT   & 23662 & 4.171 & 792  & 1.191 & 944  & 35946 & 4.449 & 845  & 1.957 & 1654 & 37172 & 4.497 & 854  & 1.996 & 1705 \\
    BHA-NOOPT & 24606 & 5.918 & 1124 & 1.281 & 1440 & 38036 & 6.008 & 1141 & 2.199 & 2510 & 39297 & 6.008 & 1141 & 2.247 & 2565 \\
    \hline
  \end{tabular}
  \label{tab:hrt}
  \vspace{4.0mm}
\end{table*}

\begin{table}[t]
  \centering
  \caption{Impact of delay constraints on the Kalyna design under the \textit{serial1col} architecture.}
  \vspace{-3mm}
  \footnotesize
  \begin{tabular}{|c|c|c|c|c|}
    \hline
    area & delay & latency & power & energy \\ 
    \hline \hline
      23662 & 4.171 & 792 & 1.191 & 944 \\
      24103 & 2.053 & 390 & 1.143 & 446 \\
      24582 & 1.491 & 283 & 1.194 & 338 \\
      28479 & 1.228 & 233 & 1.291 & 301 \\
      31756 & 1.083 & 205 & 1.514 & 312 \\
      35010 & 1.029 & 195 & 1.671 & 327 \\
    \hline
  \end{tabular}
  \label{tab:mfreq}
  \vspace{-6mm}
\end{table}

\begin{table*}[t]
	\centering
	\caption{Gate-level synthesis results of the \textit{serial1col} implementations.}
	\vspace{-3mm}
	\footnotesize
	\begin{tabular}{c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|@{\hskip3pt}c@{\hskip3pt}|}
		\hline
		\multicolumn{5}{c|}{\textit{serial1col\_oneon}} & \multicolumn{5}{c|}{\textit{serial1col\_allon}} & \multicolumn{5}{c|}{\textit{serial1col\_rndon}} \\ 
		\hline
		area & delay & latency & power & energy & area & delay & latency & power & energy & area & delay & latency & power & energy\\
		\hline \hline
		23662 & 4.171 & 792  & 1.191 & 944  & 23589 & 4.204 & 190 & 798 & 1.625 & 1298 & 23914 & 4.203 & 190 & 798 & 2.736 & 2185 \\
		\hline
	\end{tabular}
	\label{tab:hrt}
	\vspace{-4mm}
\end{table*}


